Turbulence measurements from HI absorption spectra

We use the millennium Arecibo 21 cm absorption-line survey measurements to examine the issue of the non-thermal contribution to the observed Galactic HI line widths. If we assume a simple, constant pressure model for the HI in the Galaxy, we find that the non-thermal contribution to the line width, v_{nt} scales as v^2_{nt} \propto l^{\alpha}, for v_{nt} larger than \sim 0.7 km s^{-1}. Here l is a derived length scale and \alpha \sim 0.7 \pm 0.1. This is consistent with what one would expect from a turbulent medium with a Kolmogorov scaling. Such a scaling is also predicted by theoretical models and numerical simulations of turbulence in a magnetized medium. For non-thermal line widths narrower than \sim 0.7 km s^{-1}, this scaling breaks down, and we find that the likely reason is ambiguities arising from Gaussian decomposition of intrinsically narrow, blended lines. We use the above estimate of the non-thermal contribution to the line width to determine corrected HI kinetic temperature. The new limits that we obtain imply that a significantly smaller (\sim 40% as opposed to 60%) fraction of the atomic interstellar medium in our Galaxy is in the warm neutral medium phase.

==> readme <==
%auto-ignore

This file contain information regarding the paper "Turbulence measurements from HI absorption spectra"
Authors: Nirupam Roy, Leshma Peedikakkandy, Jayaram N. Chengalur

The contact details of the first author are as follows
Nirupam Roy
email  : nirupam@ncra.tifr.res.in
    
Comments: 5 pages, 7 figures. Corrected typos. Accepted for publication in 
MNRAS Letters. The definitive version will be available at 
http://www.blackwell-synergy.com .   

Abstract: We use the millennium Arecibo 21 cm absorption-line survey 
measurements to examine the issue of the non-thermal contribution to the 
observed Galactic HI line widths. If we assume a simple, constant pressure 
model for the HI in the Galaxy, we find that the non-thermal contribution to 
the line width, v_{nt} scales as v^2_{nt} \propto l^{\alpha}, for v_{nt} 
larger than \sim 0.7 km s^{-1}. Here l is a derived length scale and \alpha 
\sim 0.7 \pm 0.1. This is consistent with what one would expect from a 
turbulent medium with a Kolmogorov scaling. Such a scaling is also predicted 
by theoretical models and numerical simulations of turbulence in a magnetized 
medium. For non-thermal line widths narrower than \sim 0.7 km s^{-1}, this 
scaling breaks down, and we find that the likely reason is ambiguities arising 
from Gaussian decomposition of intrinsically narrow, blended lines. We use the 
above estimate of the non-thermal contribution to the line width to determine 
corrected HI kinetic temperature. The new limits that we obtain imply that a 
significantly smaller (\sim 40% as opposed to 60%) fraction of the atomic 
interstellar medium in our Galaxy is in the warm neutral medium phase.                                                                      

 The compressed tar file "turhi.tar.gz" contain the following files:
 readme            This file
 mn2e.cls          MNRAS document class file
 mn2e.bst          MNRAS Bibliography style file
 turhi.tex         TEX file of the paper 
 nhts.eps          Figure 1 in the paper
 vnlt.eps          Figure 2 in the paper
 vntl1.eps         Figure 3 in the paper
 thst.eps          Figure 4 in the paper
 histat.eps        Figure 5 in the paper
 thstc.eps         Figure 6 in the paper
 lhst.eps          Figure 7 in the paper                                   

